SIDA: Social Media Image Deepfake Detection, Localization and Explanation with Large Multimodal Model

The rapid advancement of generative models in creating highly realistic images poses substantial risks for misinformation dissemination. For instance, a synthetic image, when shared on social media, can mislead extensive audiences and erode trust in digital content, resulting in severe repercussions. Despite some progress, academia has not yet created a large and diversified deepfake detection dataset for social media, nor has it devised an effective solution to address this issue. In this paper, we introduce the Social media Image Detection dataSet (SID-Set), which offers three key advantages: (1) extensive volume, featuring 300K AI-generated/tampered and authentic images with comprehensive annotations, (2) broad diversity, encompassing fully synthetic and tampered images across various classes, and (3) elevated realism, with images that are predominantly indistinguishable from genuine ones through mere visual inspection. Furthermore, leveraging the exceptional capabilities of large multimodal models, we propose a new image deepfake detection, localization, and explanation framework, named SIDA (Social media Image Detection, localization, and explanation Assistant). SIDA not only discerns the authenticity of images, but also delineates tampered regions through mask prediction and provides textual explanations of the model's judgment criteria. Compared with state-of-the-art deepfake detection models on SID-Set and other benchmarks, extensive experiments demonstrate that SIDA achieves superior performance among diversified settings. The code, model, and dataset will be released.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/6_limitations_and_further_works.tex <==
\section{Limitations and Further Works}
\label{sec:Limitations and Further Works}
In this work, we introduce SIDA and SID-Set for deepfake detection and localization tasks in social media images. We also preliminarily verify the interpretability of VLMs in deepfake detection tasks. However, we recognize some potential limitations and will continue to optimize these in future research.
%In this work, we present SIDA and SID-Set for social media image detection and localization tasks. However, there are still some limitations that need to be addressed in the future.
\\
\textbf{Dataset Size}.
While SID-Set includes 100k fully synthetic and 100k tampered images, the complexity of real social media environments demands a larger dataset. Therefore, expanding the dataset with additional images is a crucial objective for future research. 
%Although SID-Set contains 100k fully synthetic images and 100k tampered images, a larger dataset is needed to better handle the complexity of real social media scenarios. Expanding the dataset with more images will be a key goal in future work.
\\
\textbf{Data Domain}.
Other methods often generate social media images that lack authenticity or are easily identifiable. Consequently, we used only FLUX to generate fake images due to its superior quality. However, depending exclusively on one method may lead to issues of data skew, although this was not significantly evident in our experiments. Such skew could potentially impair performance on diverse datasets. Moving forward, we plan to explore additional generative methods and integrate various other generation techniques to produce a more varied and higher-quality set of images.
%We used FLUX to generate fake images due to its high quality. However, relying on a single generation method may lead to data domain shifts, which could decrease performance across diverse data. We plan to explore additional generative approaches to create more varied images in the future.
\\
\textbf{Localization Results}.
Although SIDA demonstrates relatively strong performance on our dataset, there is still room for improvement. Certain tampered regions are not reliably detected, underscoring the need for further advancements.
%Although SIDA performs well on our dataset, there is still room for improvement. Some tampered regions remain unrecognizable, highlighting the need for further advancements. We intend to investigate how to better leverage LLMs for deepfake detection and localization tasks to enhance SIDA's performance.

